Diffusion Spectral Representation for Reinforcement Learning

Diffusion-based models have achieved notable empirical successes in reinforcement learning (RL) due to their expressiveness in modeling complex distributions. Despite existing methods being promising, the key challenge of extending existing methods for broader real-world applications lies in the computational cost at inference time, i.e., sampling from a diffusion model is considerably slow as it often requires tens to hundreds of iterations to generate even one sample. To circumvent this issue, we propose to leverage the flexibility of diffusion models for RL from a representation learning perspective. In particular, by exploiting the connection between diffusion models and energy-based models, we develop Diffusion Spectral Representation (Diff-SR), a coherent algorithm framework that enables extracting sufficient representations for value functions in Markov decision processes (MDP) and partially observable Markov decision processes (POMDP). We further demonstrate how Diff-SR facilitates efficient policy optimization and practical algorithms while explicitly bypassing the difficulty and inference cost of sampling from the diffusion model. Finally, we provide comprehensive empirical studies to verify the benefits of Diff-SR in delivering robust and advantageous performance across various benchmarks with both fully and partially observable settings.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} 
    \item[] Justification: The main claims are that (1) by exploiting the energy-based model view of the diffusion model, we develop an algorithm to learn a latent variable representation of the transition function (Section~\ref{subsec:linear_repr}) and (2) we demonstrate that said representation is sufficiently expressive to linearly represent the value function, paving the way for efficient planning and exploration, circumventing the need for sample generation from the diffusion model, and thus, avoiding the inference costs associated with prior diffusion-based methods (Section~\ref{subsec:planning_exploration}). 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} %, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the assumptions in the derivations and experiments. We also address limitations in the conclusion. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide full sets of assumptions in the main text body and if an additional proof is required, we supplement in the Appendix. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide a representation training algorithm implementation description in Algorithm~\ref{alg:online} and full online pipeline implementation in Algorithm~\ref{alg:training}. We provide experimental setup and procedures in~\ref{sec:exp}. We also provide additional implementation details and hyperparameter set in~\ref{appendix:implementation}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}%\answerNo{} %, or \answerNA{}.
    \item[] Justification: We have
included all experimental details; code is released on our website.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including h   ow to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide full algorithm description in Algorithm~\ref{alg:training} and ~\ref{alg:online}, and experiment details in Appendix~\ref{appendix:implementation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: For all experimental results, we run over multiple random seeds and provide error bars for each result.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} %, \answerNo{}, or \answerNA{}.
    \item[] Justification: We run our experiments on a Quadro RTX 6000 and provide run time results. Our experiments can be done on standard graphics cards and do not require excessive computational capabilities. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We acknowledge and affirm the importance of the NeurIPS Code of Ethics. We have carefully considered the ethical implications of our work throughout the research and development process. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: We develop reinforcement learning algorithms with broad applicability. These algorithms can be used for diverse applications, some with positive outcomes and others with potential risks. Our contribution lies in the general method, not its specific use case.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: This project does not use data or models that have a high risk for misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer:  \answerYes{} 
    \item[] Justification: We have credited creators and original owners of assets (e.g., code, data, models) used in the paper. The license and terms of use are explicitly mentioned and properly respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The assets are not released at this time. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer:  \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not involve IRB approval, crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> method_new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-2mm}
\section{\algname for Efficient Reinforcement Learning}\label{sec:diff_repr}
\vspace{-2mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

It is well known that the generation procedure of diffusion models becomes the major barrier for real-world application, especially in RL. 
Moreover, the complicated generation procedure makes the uncertainty estimation for exploration intractable. The spectral representation $\phi^*(s, a)$ provides an efficient way for planning and exploration, as illustrated in~\secref{sec:prelim}, which inspires our \emph{\algname~(\algabb)} for RL, as our answer to the motivational question. As we will demonstrate below, the representation view of diffusion model enjoys the flexibility and also enables efficient planning and exploration, while directly bypasses the cost of sampling. For simplicity, we introduce~\algabb in MDP setting in the main text. However, the proposed \algabb is also applicable for POMDPs as shown  in~\appref{appendix:pomdp}. 
We first illustrate the inherent challenges of applying diffusion models for representation learning in RL. 
%thereby highlighting our technical contributions.



%%%%%%%%---------------------------------------------------
\vspace{-2mm}
\subsection{An Impossible Reduction to LV-Rep~\citep{ren2022latent}}\label{subsec:difficulty}
\vspace{-2mm}
%%%%%%%%---------------------------------------------------

% \Bo{
% discussion about the non-trivality of diffusion repr (LV-rep is not directly applicable)
% }

In the latent variable representation~(LV-Rep)~\citep{ren2022latent}, the latent variable model is exploited for spectral representation $\phi^*\rbr{s,a}$ in~\eqref{eq:svd}, by which the arbitrary state-value function is linearly represented, and thus, enable efficient planning and exploration. 
Specifically, in the LV-Rep, one considers the factorization of dynamics as
\begin{equation}\label{eq:lv_rep}
    \PP(s'|s, a) = \int p(z|s, a)p(s'|z)dz = \inner{p(z|s, a)}{p(s'|z)}_{L_2}.
\end{equation}
By recognizing the connection between~\eqref{eq:lv_rep} and SVD of transition operator~\eqref{eq:svd}, the ELBO learned latent variable model $p(z|s, a)$ can be used as $\phi^*(s, a)$ for linearly representing the $Q^\pi$-function for arbitrary policy $\pi$. 
% Inspired by the empirical successes and theoretical advantages of LV-Rep, we would like to extract the similar sufficient linear representations, but from diffusion models, which is more flexible. 

Since the diffusion model can be recast as a special type of latent variable model~\citep{ho2020denoising}, the first straightforward idea is built upon the LV-Rep with diffusion model for $p(z|s, a)$. We consider the {conditional forward process} as 
\[
p(z_i|z_{i-1}, s, a), \quad \forall i=1,\ldots, k, 
\] 
with $z_0 = s'$, which conditioning on $(s, a)$ perturbs $z_{i-1}$ with Gaussian noises. 
Then, following the definition of the diffusion model, the {backward model} will be set as
\begin{equation}
    q(z_{i-1}|z_i, s, a), \quad \forall i=0,\ldots, k, 
\end{equation}
which are also Gaussians converting the noise to next state. Thus, we have the dynamics model as
\begin{equation}\label{eq:diff_dynamics}
    \PP(s'|s, a) = \int \prod_{i=2}^{k} q(z_{i-1}|z_i, s, a) q(s'|z_1, s, a)d \cbr{z_i}_{i=1}^k.
\end{equation}
Indeed, Equation~\eqref{eq:diff_dynamics} converts the diffusion model to a latent variable model for the dynamic transition model. However, due to the dependency of $(s, a)$ in $q(s'|z_1, s, a)$, which induces extra undesirable dependency of $(s, a)$ into $\mu(s')$ in~\eqref{eq:svd}, the factorization provided by the diffusion model cannot linearly represent the $Q^\pi$-function,  
% Therefore, the it cannot provide the sufficient linear representation for RL as LV-Rep. 
making the LV-Rep reduction from diffusion models impossible. 

%%%%%%%%---------------------------------------------------
\vspace{-2mm}
\subsection{\algname from Energy-based View}\label{subsec:linear_repr}
\vspace{-2mm}
%%%%%%%%---------------------------------------------------

% \Bo{energy-based view of diffusion model}

% With the understanding of the difficulty in converting diffusion to LV-Rep. 
We introduce key observations to connect the dots between the diffusion model and spectral representation from transition in~\eqref{eq:svd} from the energy-based model~(EBM) view for a practical algorithm.
% , \ie, 
% \begin{itemize}[leftmargin=*, nosep]
%     \item[{\bf i)},] the energy-based model~(EBM) view of spectral representation~\citep{ren2022free,nachum2021provable}; 
%     and
%     \item[{\bf ii)},] the connection between EBMs and diffusion models~\citep{song2019generative} with Tweedie's identity~\citep{efron2011tweedie}.
% \end{itemize} 
%
\vspace{-2mm}
\paragraph{Spectral Representation from EBMs.} We apply the EBM for transition operator, \ie, 
%\vspace{-2mm}
\begin{equation}\label{eq:factor_ebm}
    \PP(s'|s, a) = \exp\rbr{\psi(s, a)^\top \nu\rbr{s'} - \log Z\rbr{s, a}},\, Z\rbr{s, a} = \int \exp\rbr{\psi(s, a)^\top \nu\rbr{s'}} \dif s'.
\end{equation}
To recover the SVD factorization of $\PP\rbr{s'|s, a}$ from~\eqref{eq:factor_ebm}, we exploit the random Fourier features. Specifically, by simple algebra manipulation, 
\[
\psi(s, a)^\top \nu\rbr{s'} = -\frac{1}{2}\rbr{\nbr{\psi\rbr{s, a} - \nu\rbr{s'}}^2 + \nbr{\psi\rbr{s, a}}^2 + \nbr{\nu\rbr{s'}}^2},
\]
we obtain the quadratic potential function, leading to 
\begin{equation}\label{eq:quadratic_ebm}
\textstyle
     \PP(s'|s, a) \propto \exp\rbr{{\nbr{\psi\rbr{s, a}}^2}/{2}}\exp\rbr{-{\nbr{\psi\rbr{s, a} - \nu\rbr{s'}}^2}/{2}}\exp\rbr{{\nbr{\nu\rbr{s'}}^2}/{2}}. 
\end{equation} 
The term $\exp\rbr{-\frac{\nbr{\psi\rbr{s, a} - \nu\rbr{s'}}^2}{2}}$ is the Gaussian kernel, for which we apply the random Fourier feature~\citep{rahimi2007random,dai2014scalable} and obtain the spectral decomposition of~\eqref{eq:factor_ebm},  
\begin{equation}\label{eq:spectral_ebm}
     \PP(s'|s, a) =  \inner{\phi_\omega\rbr{s, a}}{\mu_\omega\rbr{s'}}_{\Ncal\rbr{\omega}},
\end{equation}
where $\omega\sim \Ncal\rbr{0, \Ib}$, and
\begin{align}\label{eq:ebm_repr}
    \textstyle
    \phi_\omega\rbr{s, a}& = \exp\rbr{-\ib \omega^\top \psi\rbr{s, a}}\exp\rbr{{\nbr{\psi\rbr{s, a}}^2}/{2} - \log Z\rbr{s, a}}, \\
    \mu_\omega\rbr{s, a} &= \exp\rbr{-\ib\omega^\top \nu\rbr{s'}}\exp\rbr{{\nbr{\nu\rbr{s'}}^2}/{2}}.
\end{align}
This bridges the factorized EBMs~\eqref{eq:factor_ebm} to SVD, offering a spectral representation that facilitates efficient planning and exploration for linearly represented $Q$-functions, as will be shown subsequently.%in~\secref{subsec:planning_exploration}.

Exploiting the random feature to connect EBMs to spectral representation for RL was first proposed by~\citep{ren2022free,nachum2021provable}, where only Gaussian dynamics $p(s'|s, a)$ has been considered with tractable closed-formed $Z\rbr{s,a}$ and the MLE reducing to regression. 
Equation~\eqref{eq:factor_ebm} is also discussed in ~\citep{zhang2023energy,ouhamma2023bilinear,zheng2022optimistic} with UCB for exploration. However, due to the notorious difficulty in optimization of MLE of EBM caused by the intractability of $Z\rbr{s, a}$, discussed in~\citep{zhang2022making},
only special cases of~\eqref{eq:factor_ebm} have been practically implemented. 
% which as discussed in~\citep{ren2022latent} is a Gaussian latent variable model. 
How to exploit the flexibility of general EBMs in~\eqref{eq:factor_ebm} with efficient learning in practice is still open.

\vspace{-2mm}
\paragraph{Tweedie's Identity for EBM Diffusion.}
We revisit the EBM understanding of the diffusion model, which not only justifies the flexibility of diffusion models, but more importantly, paves the path for efficient learning of spectral representation~\eqref{eq:ebm_repr} through Tweedie's identity for diffusion models.

Given $\rbr{s, a}$, we consider the samples from dynamics $s'\sim\PP(s'|s, a)$ is perturbed with Gaussian noise, \ie,
% $\stil' = \sqrt{1 - \beta}s' + \sqrt{\beta}\epsilon$ with $\epsilon\sim \Ncal\rbr{0, \sigma^2I}$, which induces the perturbation
% \vspace{-2mm}
% \begin{equation*}
$\PP(\stil'|s'; \beta) = \Ncal\rbr{\sqrt{1 - \beta}s', \beta\sigma^2 I}$.
% \end{equation*}
Then, we parametrize the corrupted dynamics as
\begin{equation}\label{eq:corrupted_ebm}
    \PP(\stil'|s, a; \beta) = \int \PP(\stil' | s'; \beta) \PP(s'|s, a)ds' \propto  \exp\rbr{\psi\rbr{s, a}^\top \nu(\stil', \beta) },
\end{equation}
in which $\psi\rbr{s, a}$ is shared across all noise levels $\beta$, and 
$\PP(\stil'|s, a; \alpha) \rightarrow \PP(s'|s, a)$ with $\stil' \rightarrow s'$, as $\beta\rightarrow 0$, there is no noise corruption on $s'$. 
%
% and $A\rbr{s, a;\alpha} \defeq \log \int \exp\rbr{\phi\rbr{s, a}^\top \mu(\stil', \alpha)} d\stil'$
% where we have 
% \begin{align}
% p(\stil'|s, a; 0) = p(s'|s, a), \quad  \text{if } \alpha = 0.
%   % \begin{cases}
%   %   p(s'|s, a)       & \quad \text{if } \alpha = 0\\
%   %   p(\stil'|s, a)  & \quad \text{o.t.  }
%   % \end{cases}
% \end{align}
%
% \vspace{-1mm}
\begin{proposition}[Tweedie's Identity~\citep{efron2011tweedie}]
% For arbitrary $\beta$ and $\epsilon\sim \Ncal\rbr{0, I}$, $\stil' = \sqrt{1 - \beta}s + \sqrt{\beta}\epsilon$, 
For arbitrary corruption $\PP\rbr{\stil'|s'; \beta}$ and $\beta$ in $\PP\rbr{\stil'|s, a; \beta}$, we have 
\begin{equation}\label{eq:generali_tweedie}
    \nabla_{\stil'} \log \PP(\stil'|s, a; \beta) = \EE_{\PP(s'|\stil',s, a; \beta)}\sbr{\nabla_{\stil'} \log \PP(\stil' | s'; \beta)}.
\end{equation}
\end{proposition}
\vspace{-2mm}
This can be easily verified by simple calculation, \ie, 
\begin{align}
    &\nabla_{\stil'}\log \PP(\stil'|s, a; \beta) = \frac{\nabla_{\stil'} \PP(\stil'|s, a; \beta) }{\PP(\stil'|s, a; \beta) } = \frac{\nabla_{\stil'} \int \PP(\stil' | s'; \beta) \PP(s'|s, a)ds' }{\PP(\stil'|s, a; \beta) } \nonumber\\
    &= \int \frac{\nabla_{\stil'} \log \PP(\stil' | s'; \beta)\PP(\stil' | s'; \beta) \PP(s'|s, a) }{\PP(\stil'|s, a; \beta)} ds' = \EE_{\PP(s'|\stil',s, a; \beta)}\sbr{\nabla_{\stil'} \log \PP(\stil' | s'; \beta)},
\end{align}


For Gaussian perturbation with~\eqref{eq:corrupted_ebm}, Tweedie's identity~\eqref{eq:generali_tweedie} is applied as
\begin{align}\label{eq:gauss_tweedie}
     \psi\rbr{s, a}^\top \nabla_{\stil'}\nu\rbr{\stil', \beta} &= \EE_{\PP(s'|\stil', s, a; \beta)}\sbr{\frac{\sqrt{1 - \beta} s' - \stil'}{\beta\sigma^2}} \nonumber
     \\
     \Rightarrow \stil' + \beta\sigma^2 \psi\rbr{s, a}^\top \nabla_{\stil'}\nu\rbr{\stil', \beta} & = \sqrt{1 - \beta} \EE_{\PP(s'|\stil',s, a; \beta)}\sbr{s'}.
\end{align}
Let $\zeta\rbr{\stil'; \beta} = \nabla_{\stil'}\nu\rbr{\stil', \beta}$, we can learn $\psi\rbr{s, a}$ and $\zeta\rbr{\stil'; \beta}$
%and the score function $\zeta\rbr{\stil'; \beta}$, 
by matching both sides of~\eqref{eq:gauss_tweedie}, 
\begin{equation}\label{eq:intermedia}
    \min_{\psi, \zeta} \,\,\EE_\beta\EE_{(s, a, \stil')}\sbr{\nbr{\stil' + \beta\sigma^2 \psi\rbr{s, a}^\top \zeta\rbr{\stil', \beta}  - \sqrt{1 - \beta}\EE_{\PP\rbr{s'|\stil', s, a; \beta}}\sbr{ s' }}^2}  
\end{equation}
which shares the same optimum of 
\begin{equation}\label{eq:diff_learn}
     \min_{\psi, \zeta} \,\,\ell_{\text{diff}}\rbr{\psi, \zeta}\defeq \EE_\beta\EE_{(s, a, \stil', s')}\sbr{\nbr{\stil' + \beta\sigma^2 \psi\rbr{s, a}^\top \zeta\rbr{\stil', \beta}  - \sqrt{1 - \beta} s'}^2}. 
     % + \underbrace{\EE_\beta\EE_{(s, a, \stil', s')}\sbr{\rbr{1 - \beta}\nbr{s'  - \EE_{\PP\rbr{s'|\stil', s, a; \beta}}\sbr{s'}}^2}}_{\texttt{constant}}
\end{equation}
The equivalence of~\eqref{eq:intermedia} and~\eqref{eq:diff_learn} is provided in~\appref{appendix:details}.

%\chenjun{Maybe add some discussion here and emphasize that we do not sample from the diffusion model? }\Bo{I thought we can do this in the planning section.}\chenjun{done}


\vspace{-2mm}
\paragraph{Normalized Finite-dimensional Approximation.}
The optimization described by~\eqref{eq:diff_learn} characterizes the loss associated with specific parametrized diffusion models, employing the score function $\psi\rbr{s, a}^\top\zeta\rbr{\stil', \beta}$. 
This formulation enables the estimation of the score function up to a normalization term known as the partition function. In the context of generating samples, the score function suffices to drive the reverse Markov chain process. However, when engaging approximating value function with the random feature $\phi_\omega$ defined in \eqref{eq:ebm_repr}, the partition function is indispensable. 
But with our parametrization of the score function where $\zeta\rbr{\stil',\beta} = \nabla_{\stil'}\nu\rbr{\stil', \beta}$, the computation of the partition function becomes increasingly challenging. Furthermore, the random feature $\phi_\omega(s, a)$ is only conceptual with infinite dimensions with $\omega\sim \Ncal\rbr{0, I}$.  


To obtain a tractable finite-dimensional representation without explicit partition function calculation, we propose a reparameterization for $\phi_\omega(s, a)$ with some neural network upon $\psi\rbr{s, a}$, while satisfying the spectral property. 
Specifically, in the definition of $\phi_\omega\rbr{s, a}$ in~\eqref{eq:spectral_ebm}, it contains Fourier basis $\exp\rbr{-\ib \omega^\top \psi\rbr{s, a}}$, suggesting the use of $\sin$-functions~\citep{rahimi2007random} upon $\psi\rbr{s, a}$. Meanwhile, it also contains a product with quadratic term $\exp (\nbr{\psi\rbr{s, a}}^2)$, suggesting the additional nonlinearity. Therefore, 
we consider the finite-dimensional neural network $\phi_{\theta}\rbr{s, a} = \texttt{elu}\rbr{W_2\sin\rbr{W_1^\top \psi\rbr{s, a}}}\in \RR^d$ with learnable parameters $\theta = \rbr{W_1, W_2}$, to approximate the infinite-dimensional $\phi_\omega\rbr{s, a}$ with $\omega\sim \Ncal\rbr{0, I}$.


Recall the fact that for $\forall (s, a)\in \Scal\times\Acal$, we have
\begin{align*}
    \inner{\phi_\omega\rbr{s, a}}{\phi_\omega\rbr{s, a}}_{\Ncal\rbr{\omega}} 
    % &= \frac{\exp\rbr{\nbr{\psi\rbr{s, a}}^2}}{Z^2\rbr{s, a}}\underbrace{\int \exp\rbr{\ib \omega^\top (\psi\rbr{s, a}  - \psi\rbr{s, a}} \Ncal\rbr{\omega}) d\omega}_{ 1},\\
    =  \exp\rbr{\nbr{\psi\rbr{s, a}}^2 - 2\log Z\rbr{s, a}},
\end{align*}
which implies the relationship 
\begin{equation}
    Z\rbr{s, a} =\exp\rbr{\frac{\nbr{\psi\rbr{s, a}}^2 - \log\nbr{\phi_\omega\rbr{s, a}}^2}{2}}. 
\end{equation}
We follow the suggestion in~\citep{zhang2023energy,zhang2022making} that constrains $Z\rbr{s, a} = 1$, $\forall (s, a)\in \Scal\times \Acal$ for identifiability, which induces the regularization 
\begin{equation}
    \ell_{\text{norm}}\rbr{\psi, \theta} = \EE_{s, a}\sbr{\rbr{\nbr{\psi\rbr{s, a}}^2 - \log\nbr{\phi_\omega\rbr{s, a}}^2}^2}. 
\end{equation}


% Recall the fact that the~\algabb plays as the SVD of transition operator, this observation motivates the orthormal regularization during optimization for $\phi_\theta\rbr{s, a}$. 
% We employ the regularization proposed in \citep{wu2018laplacian},
% \begin{align*}
%     \textstyle
%     \ell_{\text{orth}}\rbr{\psi, \theta} &= \sum_{i,j}\rbr{\EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a}} - \delta_{ij}}^2 \\
%     % &= \sum_{i,j}\EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a} - \delta_{ij}} \EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a} - \delta_{ij}} \\
%     &=\sum_{ij} \EE_{\rbr{s, a}_1, \rbr{s, a}_2 }\sbr{\rbr{\phi_\theta^i\rbr{s_1, a_1}\phi_\theta^j\rbr{s_1, a_1} - \delta_{ij}}\rbr{\phi_\theta^i\rbr{s_2, a_2}\phi_\theta^j\rbr{s_2, a_2} - \delta_{ij}}},
% \end{align*}
% where $\phi_\theta^i\rbr{s, a}$ denotes the $i$-th dimension of $\phi_\theta\rbr{s, a}$, and $\delta_{ij} = 1$ if $i=j$, and $\delta_{ij} = 0$ otherwise. 

Together with the normalized regularization with score matching, we obtain the loss for~\algabb learning, \ie, 
%\vspace{-2mm}
\begin{equation}\label{eq:diff-rep-objective}
    \min_{\psi, \zeta, \theta}\,\, \ell_{\text{diff}}\rbr{\psi, \zeta} + \lambda \ell_{\text{orth}}\rbr{\psi, \theta},
\end{equation}
with $\lambda >0$. It extracts $\phi_\theta{\rbr{s, a}}$ for representing $Q$-function in planning in~\secref{subsec:planning_exploration}. Algorithm~\ref{alg:training} presents pseudocode for learning diffusion representations. 


\vspace{-2mm}
\paragraph{Remark (Connection to sufficient dimension reduction~\citep{sasaki2018neural}):} The theoretical properties of $\psi\rbr{s, a}$ in the potential function in EBMs~\eqref{eq:factor_ebm} have been investigated in~\citep{sasaki2018neural}. Concretely, the factroization parametrization is actually universal approximation capable. 
%, even with factorization in potential function. 
Moreover, the $\psi\rbr{s, a}$ also constructs an implementation of sufficient dimension reduction~\citep{fukumizu2009kernel}, \ie, given $\psi\rbr{s, a}$, we have $\PP(s'|s, a) = \PP\rbr{s'|\psi\rbr{s, a}}$, or equivalently $s'\perp (s, a)|\psi\rbr{s, a}$. 
These two properties clearly justified the expressiveness and sufficiency of the learned $\psi\rbr{s, a}$. However, the $\psi\rbr{s, a}$ in~\citep{sasaki2018neural} is not learned from our diffusion-based criterion, and $\psi\rbr{s, a}$ is only estimated up to the partition function $Z(s, a)$, which may not directly applicable for planning and exploration in RL as we discussed below.


\begin{algorithm}[t]
\caption{\algname~(\algabb) Training}
\label{alg:training}
\begin{algorithmic}[1]
\State \textbf{Input:} representation networks $\psi, \zeta, \theta$, noise levels $\{\beta^k\}_{k=1}^T$, replay buffer $\mathcal{D}$

% batch size $n$, Number of noise terms $T$, Training cumulative product noise terms $ \{ \alpha_t \}_{t = 1}^{t = T}$, Sigma scale factor $ \omega$,   
% \State \textbf{Initialize:} $\phi (s, a)  \rightarrow z, \nabla_{\tilde{s}'} \mu( \tilde{s}',  \alpha ) \rightarrow s \times z $,  Replay buffer $\mathcal{B}$
\For{update step $= 1, 2, ..., N_{\text{rep}}$}
\State Sample a batch of $n$ transitions $\{(s_i, a_i, s_i')\}_{i=1}^n\sim\mathcal{B}$
\State Sample noise schedules for each transition $\{\beta_i\}_{i=1}^n\sim \text{Uniform}(\beta^1, \beta^2, \ldots, \beta^T)$
\State Corrupt the next states $\tilde{s}_i'\leftarrow \sqrt{1-\beta_i}s_i'+\sqrt{\beta_i}\epsilon_i$, where $\epsilon_i\sim\mathcal{N}(0, \sigma^2I)$
\State Optimize $\psi, \zeta, \theta$ via gradient descent by minimizing Eq~\eqref{eq:diff-rep-objective}
\EndFor

\State \textbf{Return} $\psi, \zeta$
% \For{environment step $ = 1 \textbf{ to }$ Evaluation Length}
%     \State $ \{ (s, a, s')  \}_n \sim \mathcal{B}$  \Comment{Sample $n$ transitions from $\mathcal{B}$}
%     \State $\alpha \sim \{\alpha_t \}_{t = 1}^{t = T}$ \Comment{Sample noise terms of shape $n \times \dim(s)$ from $T$ noise terms}
%     \State $ \epsilon  \sim \mathcal{N}(0,\omega I_n  )$ \Comment{Sample Normal distribution with variance scaled by $\omega$}
%     \State $\tilde{s}'   = \sqrt{ \alpha  } \cdot s'  + \sqrt{ 1. -  \alpha  } \cdot  \epsilon   $ \Comment{Calculate next state batch perturbed }
%     \State $\min_{\phi, \mu} \mathbb{E}_\alpha \mathbb{E}_\mathcal{D} \left[  ||  \tilde{s}' + (1 - \alpha)^2 \sigma^2  \phi(s, a)^T \nabla_{\tilde{s}'} \mu(\tilde{s}', \alpha)   - \alpha s'||^2  \right]$ \Comment{Take feature optimizer step on diffusion loss}
% \EndFor

% \State \textbf{Return} $\phi (s, a), \nabla_{\tilde{s}'} \mu( \tilde{s}',  \alpha )$.
\end{algorithmic}
\end{algorithm}



\iffalse

To avoid the explicit partition function calculation, we notice that in~\eqref{eq:spectral_ebm}, after the random feature over $\psi\rbr{s, a}$, the obtained feature $\phi_\omega\rbr{s, a}$ in~\eqref{eq:ebm_repr} plays as spectral factorization of transition operator. This inspires us to add orthonormal constraints on the reparametrized $\phi_{\theta}\rbr{s, a} = \texttt{relu}\rbr{W_2\sin\rbr{W_1^\top \psi\rbr{s, a}}}$ with $\theta = \rbr{W_1, W_2}$, which leads to the regularization pushing for orthonomal over $\phi_\theta\rbr{s, a}$ ~\citep{wu2018laplacian}, 
\begin{align*}
    \textstyle
    \ell_{\text{orth}}\rbr{\psi, \theta} &= \sum_{i,j}\rbr{\EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a}} - \delta_{ij}}^2 \\
    % &= \sum_{i,j}\EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a} - \delta_{ij}} \EE_{s, a}\sbr{\phi_\theta^i\rbr{s, a}\phi_\theta^j\rbr{s, a} - \delta_{ij}} \\
    &=\sum_{ij} \EE_{\rbr{s, a}_1, \rbr{s, a}_2 }\sbr{\rbr{\phi_\theta^i\rbr{s_1, a_1}\phi_\theta^j\rbr{s_1, a_1} - \delta_{ij}}\rbr{\phi_\theta^i\rbr{s_2, a_2}\phi_\theta^j\rbr{s_2, a_2} - \delta_{ij}}},
\end{align*}
where $\phi_\theta^i\rbr{s, a}$ denotes the $i$-th dimension in the output of $\phi_\theta\rbr{s, a}$, and $\delta_ij = 1$ if $i=j$, otherwise $0$. 
We select the two-layer MLP for $\phi_\theta\rbr{s, a}$ with $\sin$-activation function by the observation that $\phi_\omega\rbr{s, a}$ in~\eqref{eq:ebm_repr} contains Fourier basis $\exp\rbr{-\ib \omega^\top \psi\rbr{s, a}}$ and quadratic term $\exp\rbr{\nbr{\psi\rbr{s, a}}^2}$. 

\fi



%%%%%%%%---------------------------------------------------
\vspace{-2mm}
\subsection{Policy Optimization with Diffusion Spectral Representation}\label{subsec:planning_exploration}
\vspace{-2mm}
%%%%%%%%---------------------------------------------------

% The optimization described by~\eqref{eq:diff_learn} characterizes the loss associated with specific parametrized diffusion models, employing the score function $\psi\rbr{s, a}^\top\zeta\rbr{\stil', \beta}$. 
% This formulation enables the estimation of the score function up to a normalization term known as the partition function. In the context of generating samples, the score function suffices to drive the reverse Markov chain process. However, when engaging approximating value function with the random feature $\phi_\omega$ defined in \eqref{eq:ebm_repr}, the partition function is indispensable. 
% But with our parametrization of the score function where $\zeta\rbr{\stil',\beta} = \nabla_{\stil'}\nu\rbr{\stil', \beta}$, the computation of the partition function becomes increasingly challenging. Furthermore, the random feature $\phi_\omega(s, a)$ is only conceptual with infinite dimensions with $\omega\sim \Ncal\rbr{0, I}$.  

% We construct \emph{\algname~(\algabb)}, a tractable finite-dimensional representation without explicit partition function calculation, by approximating $\phi_\omega(s, a)$ with some neural network upon $\psi\rbr{s, a}$. 
% % while satisfying the spectral property. 
% Specifically, in the definition of $\phi_\omega\rbr{s, a}$ in~\eqref{eq:spectral_ebm}, it contains Fourier basis $\exp\rbr{-\ib \omega^\top \psi\rbr{s, a}}$, suggesting the use of trigonometry functions~\citep{rahimi2007random} upon $\psi\rbr{s, a}$, \ie, $\sin\rbr{W_1^\top \psi\rbr{s, a}}$. Meanwhile, it also contains a product with quadratic term $\exp (\nbr{\psi\rbr{s, a}}^2)$ and partition function $Z\rbr{s, a}$, suggesting the additional nonlinearity over $\sin\rbr{W_1^\top \psi\rbr{s, a}}$. Therefore, 
% we consider the finite-dimensional neural network $\phi_{\theta}\rbr{s, a} = \texttt{elu}\rbr{W_2\sin\rbr{W_1^\top \psi\rbr{s, a}}}\in \RR^d$ with learnable parameters $\theta = \rbr{W_1, W_2}$, to approximate the infinite-dimensional $\phi_\omega\rbr{s, a}$ with $\omega\sim \Ncal\rbr{0, I}$. 

With the \algabb $\phi_\theta$ approximates the spectral decomposition of the transition function $\phi_\omega$ well, the $Q$-function can be represented as a linear function of the diffusion spectral representation $\phi_\theta$. 
Consider the following \emph{two-part} value function approximation with weight vector $\xi\in\mathbb{R}^d$, 
% \vspace{-2mm}
\begin{align}
Q_{\xi, \theta}(s,a) = \phi_\theta(s,a)^\top \xi \, 
\label{eq:diff-rep-q}
\end{align}
This approximated value function can be integrated into any model-free algorithm to facilitate policy optimization.
In particular, we update $\rbr{\xi}$ with the standard TD loss 
\begin{align}
\ell_{\text{critic}} (\xi) = \mathbb{E}_{s,a,r,s'\sim\mathcal{D}}\left[ \left( r + \gamma \mathbb{E}_{a'\sim \pi} [ Q_{\bar{\xi}, \theta}(s',a') ]  - Q_{\xi, \theta}(s,a) \right)^2 \right] \, ,
\label{eq:q-update}
\end{align}
where $\pi$ is the learning algorithm's current policy, $\bar{\xi}$ is the target network, $\mathcal{D}$ is the replay buffer. 
We apply the \emph{double Q-network trick} to stabilize training \citep{fujimoto2018addressing}.  
In particular, two weights $\xi_1, \xi_2$ are initialized and updated independently according to \eqref{eq:q-update}. 
Then the policy is updated by considering $\max_{\pi} \mathbb{E}_{s\sim \mathcal{D},a\sim\pi} [ \min_{i\in\{1,2\}} Q_{\xi_i, \theta}(s,a)]$.  
Algorithm \ref{alg:online} presents the pseudocode of online RL with \algabb. This learning framework is largely consistent with standard online reinforcement learning (RL) approaches, with the primary distinction being the incorporation of diffusion representations. As more data is collected, Line 7 specifies the update of the diffusion representation $\phi_\theta$ using Algorithm~\ref{alg:training} and the latest buffer $\mathcal{D}$. 
It is important to highlight that the value function approximation \eqref{eq:diff-rep-q} reveals another key advantage of \algabb: \emph{it explicitly eliminates the necessity to generate samples from the diffusion model}, thus bypassing the inference costs typically associated with previous diffusion-based methods. 



\vspace{-2mm}
\paragraph{Exploration with Diffusion Representation} 

Following \citep{uehara2021representation,ren2022latent}, we can similarly employ diffusion representations to implement the principle of optimism in the face of uncertainty for exploration in RL.  
We introduce additional UCB bonus in $r$ in~\eqref{eq:q-update} by 
\begin{align}
\textstyle
b(s,a) = \phi_{{\theta}}(s,a)^\top \left( \sum_{s',a'\in\mathcal{D}} \phi_{{\theta}}(s,a) \phi_{{\theta}}(s,a)^\top + \lambda I \right)^{-1} \phi_{{\theta}}(s,a) \, ,
\label{eq:bonus}
\end{align}
where $\mathcal{D}$ is a dataset of state action pairs. 
This bonus is subsequently added to the reward to facilitate exploration during the policy optimization process.




%%%%%%%%---------------------------------------------------
%\subsection{Generalization for Partially Observable RL}\label{subsec:pomdp}
%%%%%%%%---------------------------------------------------

%\Bo{==============================================}Chenjun: move to the appendix



\iffalse
\subsection{Random Fourier Feature for Infinite Dimension Representation}

As noted in Ren et al 2023, one of the challenges of latent variable representation is that for the latent feature $z$, the dimension $\dim |z|$ can be infinite. Therefore, in order to practically parameterize the $Q$ function ~\eq{eq:exp_q} with a neural network that has finite number of parameters, we need to apply the Random Fourier Feature representation. [Cite: Rahmi and Recht, Bo's paper] 

Specifically, this infinite $z$ dimension poses a challenge when we need to compute the expectation $\EE_{p^*(z|s, a)}\sbr{w^\pi(z)}$ in the $Q$ function calculation, as given by:

\begin{align}\label{eq:rff_q}
    Q_{T^*, r}^\pi(s, a) = r(s, a) + \gamma\EE_{p^*(z|s, a)}\sbr{w^\pi(z)},
\end{align}

where $w^\pi(z) = \int_{\mathcal{S}} p^*(z|s^\prime) V_{T^*, r}^\pi(s^\prime) ds^\prime$ represents the value function of the latent state. 

However, we can note that $w^\pi \in \mathcal{H}_k$, where $\mathcal{H}_k$ is a reproducing kernel Hilbert space with kernel $k$. Therefore, in order to have a tractable representation of the $Q$ function through $z$, we apply the Random Fourier Feature representation and then express $w^\pi$ as:
\begin{align*}
    w^\pi(z) = \int_{\Xi} \widetilde{w}^\pi(\xi)\psi(z; \xi) d P(\xi),
\end{align*}
where the concrete $P(\xi)$ depends on the kernel $k$. Inserting this representation of $w^\pi(z)$ into ~\eq{eq:rff_q}, we obtain the approximated representation of $Q_{T^*, r}^\pi(s, a)$ as:
\begin{align*}
Q_{T^*, r}^\pi(s,a) & = r(s, a) + \gamma\int_{\mathcal{Z}}  w^\pi(z) p^*(z|s, a) d\mu \\
& = r(s, a) + \gamma\int_\mathcal{Z} \int_\Xi \widetilde{w}(\xi) \psi(z; \xi) d P(\xi)\cdot  p^*(z|s,a) d\mu\\
& \approx r(s, a) + \frac{\gamma}{m} \sum_{i\in[m]} \widetilde{w}(\xi_i) \psi(z_i; \xi_i),
\end{align*}
which shows that we can approximate $Q_{T^* r}^\pi(s, a)$ with a linear function on top of the random feature $\varphi(s, a) = [\psi(z_i; \xi_i)]_{i\in [m]}$ where $z_i \sim p^*(z|s, a)$ and $\xi_i \sim P(\xi)$.

In practice, the allows us to use a two-layer neural network with fixed first layer weight $\xi_i$ and activation $\psi$ and trainable second layer weight $\widetilde{w} = \sbr{\widetilde{w}(\xi_i)}_{i=1}^m\in \mathbb{R}^m$ to parameterize the $Q$ function. The Random Fourier Feature allows us to utilize an infinite dimensional representation for $z$ to while maintaining a tractable parameterization for $Q$. 


% - Does not learn s' directly as part of the loss and then fits p(z | s, a, s') to p(z | s, a), rather learns score
% - Does not learn normalized probability, rather leverages unnormalized energy-based model
% - Does not need Gaussian parametric assumption, can fundamentally be multimodal
% - Does not require VAE, rather diffusion, which has all of these advantages
% -VAE's loss function has it predict the same exact as the input, therefore disincentivizing learning the underlying dynamics and rather copying state, action, next state triplets. This leads to overfitting. 
% - Much more expressive due to higher latent space - talk about parametric vs non-parametric models, especially since dimension space z is infinite rather than finite then z needs a more expressive model
% - Performs much better on multi-limb, multi-modal environments, learns dynamics distribution better. VAE needs to learn true Gaussian distribution, Diffusion is not gaussian and only needs to learn the derivative, no normalization constant. 
% - Pros: Tractability and flexibility are two conflicting objectives in generative modeling. Tractable models can be analytically evaluated and cheaply fit data (e.g. via a Gaussian or Laplace), but they cannot easily describe the structure in rich datasets. Flexible models can fit arbitrary structures in data, but evaluating, training, or sampling from these models is usually expensive. Diffusion models are both analytically tractable and flexible. 









\subsection{Energy based view}




$E_\mathbf{\theta}$ is the energy function, a nonlinear regression function with parameters $\theta$ and $Z_\theta$ is the normalizing term, which is constant with respect to $\mathbf{x}$ but is a function of $\theta$. 

In the Diff-Rep case, we consider the conditional probability $p(\tilde{s}' | s, a ; \alpha)$ as an EBM, with $- E_\theta(x) = \phi(s,a)^T \mu(\tilde{s}', \alpha)$. 

Therefore, 

\begin{align}
     p(\tilde{s}' | s, a ; \alpha) &= \dfrac{\exp(\phi(s,a)^T \mu(\tilde{s}', \alpha))  }{\int \exp(\phi(s,a)^T \mu(\tilde{s}', \alpha) )d \tilde{s}' }\\
    &= \exp  \left( \phi(s,a)^T \mu(\tilde{s}', \alpha)   - \log \int \exp(\phi(s,a)^T \mu(\tilde{s}', \alpha) )d \tilde{s}' \right)
\end{align}

We define the term $A(s, a ; \alpha) := \log \int \exp(\phi(s,a)^T \mu(\tilde{s}', \alpha) )d \tilde{s}'$, and note that A does not depend on $\tilde{s}'$, which is useful for taking the gradient later on. 


According to Song 2019, we define the score of a probability density $p(\textbf{x})$ to be defined as $\nabla_{x} \log p(x)$. This score is a vector field pointing in the direction in where the log data grows the most. The score function is easier to model and estimate than the original probability density function. 


We now consider the gradient of the log-probability of the EBM with:

\begin{align}
    \nabla_{\tilde{s}'} \log p(\tilde{s}' | s, a ; \alpha) &= \dfrac {\nabla_{\tilde{s}'}  p(\tilde{s}' | s, a ; \alpha) }{p(\tilde{s}' | s, a ; \alpha)}   
   && \text{ d(log(x)) = dx / x } \\
   &= \dfrac {\nabla_{\tilde{s}'}  \int p( \tilde{s}' | s' ; \alpha) p(s' | s, a) ds' }{p(\tilde{s}' | s, a ; \alpha)}  && \text{ direct substitution of eq. 5}  \\
   &= \int \dfrac{\nabla_{\tilde{s}'} \log  p( \tilde{s}' | s' ; \alpha) p( \tilde{s}' | s' ; \alpha) p(s' | s, a) }{p(\tilde{s}' | s, a ; \alpha)} ds'  && \text{ by sub } \nabla_{\tilde{s}'} p( \tilde{s}' | s' ; \alpha) = \nabla_{\tilde{s}'} \log p( \tilde{s}' | s' ; \alpha) p( \tilde{s}' | s' ; \alpha)   \\
   &= \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[  \nabla_{\tilde{s}'} \log  p( \tilde{s}' | s' ; \alpha)  \right]
\end{align}

To get to the next step in the derivation, we evaluate left and right terms from their original definitions, i.e  $ \nabla_{\tilde{s}'} \log p(\tilde{s}' | s, a ; \alpha)$ and $\mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[  \nabla_{\tilde{s}'} \log  p( \tilde{s}' | s' ; \alpha)  \right]$.

\begin{align}
    \nabla_{\tilde{s}'} \log p(\tilde{s}' | s, a ; \alpha) &= \nabla_{\tilde{s}'} \log \exp  \left( \phi(s,a)^T \mu(\tilde{s}', \alpha)   - A(s, a; \alpha) \right) \\
    &= \nabla_{\tilde{s}'}  \left( \phi(s,a)^T \mu(\tilde{s}', \alpha)   - A(s, a; \alpha) \right) \\
    &=  \phi(s,a)^T \nabla_{\tilde{s}'} \mu(\tilde{s}', \alpha)  
\end{align}

Similarly, 

\begin{align}
    \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[  \nabla_{\tilde{s}'} \log  p( \tilde{s}' | s' ; \alpha)  \right] &= \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ \nabla_{\tilde{s}'} \log  \mathcal{N} (\alpha s', (1 - \alpha)^2 \sigma^2 I) \right] \\
    &= \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ \dfrac{ \nabla_{\tilde{s}'}   \mathcal{N} (\alpha s', (1 - \alpha)^2 \sigma^2 I)}  {\mathcal{N} (\alpha s', (1 - \alpha)^2 \sigma^2 I ) } \right] \\
    &=  \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ \dfrac{ \nabla_{\tilde{s}'}  \exp{ \left( \frac{-1}{2}  \frac{ (\tilde{s}' - \alpha s')^2 }{ (1 - \alpha)^2 \sigma^2 } \right)  }  }{\exp{ \left(  \frac{-1}{2} \frac{ (\tilde{s}' - \alpha s')^2 }{ (1 - \alpha)^2 \sigma^2 } \right)  }} \right] \\
    &= \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ \dfrac{\alpha s' - \tilde{s}'}{ (1 - \alpha)^2 \sigma^2 } \right]
\end{align}
Since $\nabla_{\tilde{s}'} \log p(\tilde{s}' | s, a ; \alpha) = \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[  \nabla_{\tilde{s}'} \log  p( \tilde{s}' | s' ; \alpha)  \right]$, we get:

\begin{align}
    \phi(s,a)^T \nabla_{\tilde{s}'} \mu(\tilde{s}', \alpha) =  \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ \dfrac{\alpha s' - \tilde{s}'}{ (1 - \alpha)^2 \sigma^2 } \right]
\end{align}

We can move all of the non-$s'$ terms out of  $\mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)}$ and are left with the expression:

\begin{align}
   \tilde{s}' + (1 - \alpha)^2 \sigma^2 \phi(s,a)^T \nabla_{\tilde{s}'} \mu(\tilde{s}', \alpha) = \alpha \mathbb{E}_{p(s' | \tilde{s}', s, a ; \alpha)} \left[ s' \right] 
\end{align}

We can then learn the representation by regression with expectations over the noise scale and data points:

\begin{align}
    \min_{\phi, \mu} \mathbb{E}_\alpha \mathbb{E}_\mathcal{D} \left[  ||  \tilde{s}' + (1 - \alpha)^2 \sigma^2  \phi(s, a)^T \nabla_{\tilde{s}'} \mu(\tilde{s}', \alpha)   - \alpha s'||^2  \right]
\end{align}

Then, we can use the learned $\phi\rbr{s, a}$ to obtain the random feature for linear representing $Q^\pi$-function. 
\fi 

\iffalse

\subsubsection{Remark (Partition Function Regularization)}

Note that in the score-matching view of the transition dynamics, we have the case:


\begin{equation}
    \nabla_{\tilde{s}'} \log p(\tilde{s}' | s, a ; \alpha) = \nabla_{\tilde{s}'} \log \left( \frac{ p(\tilde{s}', s, a ; \alpha) }{p( s, a ; \alpha) }   \right)  = \nabla_{\tilde{s}'}  \log  p(\tilde{s}', s, a ; \alpha)  - \underbrace{\nabla_{\tilde{s}'} \log p( s, a ; \alpha)}_{\text{= 0}} =   \nabla_{\tilde{s}'}  \log  p(\tilde{s}', s, a ; \alpha) 
\end{equation}

Therefore, there can potentially be infinitely many solutions to representation $\phi(s, a)$, part of which could be solutions to the joint distribution case rather than the desired conditional dynamics distribution case. In general, score matching ensures the recovery of the potential function only up to the partition function [CITE: Zhang et all 2022 (Bo Making Linear MDPs Practical paper)].

We first consider the diffusion probability constraint
\begin{equation}\label{eq:integral}
    \int p(\stil'|s, a; \alpha) d\stil' = 1, \quad \forall (s, a)\in \Scal\times \Acal,
\end{equation}
which induces the regularizer:
\begin{equation}\label{eq:part_reg}
    \EE_{(s, a)\sim \Dcal}\sbr{\log \int p(\stil'|s, a; \alpha) d\stil' }. 
\end{equation}

In general, the integration in~\eqref{eq:integral} is difficult to compute. However, in diffusion model, we exploit the structure that 
\begin{align}    
    p(\stil'|s, a; \alpha) &= \int p(\stil'|s'; \alpha) \exp\rbr{\phi\rbr{s, a}^\top \mu\rbr{s'}} d s' \\
    &= \int \underbrace{\frac{1}{\sqrt{\rbr{2\pi\sigma^2}^k}}\exp\rbr{-\frac{\nbr{\stil' - \alpha s'}}{2(1-\alpha)^2\sigma^2}}}_{p(s', \stil', \alpha)}\exp\rbr{\phi\rbr{s, a}^\top \mu\rbr{s'}} d s' = \EE_{p(s', \stil', \alpha)}\sbr{\exp\rbr{\phi\rbr{s, a}^\top \mu\rbr{s'}}}.
\end{align}
With Monte-Carlo approximation through this formulation, we can obtain a tractable regularization if we parametrized $\mu(s', \alpha)$.  

In order to bypass the unnecessary calculation for the regularization, we consider the alternative SVD perspective. In our parametrization, we have 
\begin{equation}
    p(\stil'|s, a; \alpha) = \exp\rbr{\phi\rbr{s, a}^\top \mu\rbr{\stil', \alpha}} = \EE_{\Ncal\rbr{\omega}}\sbr{\varphi_\omega\rbr{s, a}\psi_\omega\rbr{\stil'}},
\end{equation}
where 
\begin{align}
    \varphi_\omega\rbr{s, a} &= \exp\rbr{-\frac{\nbr{\phi\rbr{s, a}}^2}{2}}\exp\rbr{j \omega^\top \phi\rbr{s, a}}, \\
    \psi_\omega\rbr{\stil'} &= \exp\rbr{-\frac{\nbr{\psi\rbr{\stil'}^2}}{2}}\exp\rbr{j \omega^\top \mu\rbr{\stil', \alpha}}.
\end{align}
This implies the $\varphi_\omega\rbr{s, a}$ and $\psi_\omega\rbr{\stil'}$ are the singular value decomposition. Therefore, we consider the regularization on $\varphi_\omega\rbr{s, a}$ as
\begin{equation}
    \EE_{\rbr{s, a}}\sbr{\varphi_{\omega_1}\rbr{s, a}\varphi_{\omega_2}\rbr{s, a}} = \delta_{\omega_1, \omega_2}, \quad \forall \rbr{s, a}\in \Scal\times\Acal. 
\end{equation}
Since the Fourier feature are naturally orthogonal, we only need to regularize for the case $\omega_1 = \omega_2$, \ie,
\begin{equation}
    \EE_{s, a}\sbr{\int p(\omega) \varphi_\omega\rbr{s, a}\varphi_\omega\rbr{s, a}d\omega } = 1 \Rightarrow \EE_{(s, a)}\sbr{\exp\rbr{\phi(s, a)^\top \phi\rbr{s, a}}} =  1.
\end{equation}

We consider the regularizer from Wu et. al 2018 [CITE] that provides a soft constraint on the orthonormality of the Laplacian eigenfunctions. In our case, we consider that

\begin{equation}
    \sum_{j,k} (\langle \varphi_{\omega_j}\rbr{s, a}, \varphi_{\omega_k}\rbr{s, a} \rangle - \delta_{jk})^2 < \epsilon.
\end{equation}

This orthonormalization regularizer is directly added to our parametrization of the $Q$ function, which follows the implementation from Ren et al. 2023. 



\subsection{Connection to Sasaki and Hyvärinen 2018}

To provide more theoretical justification as to why diffusion-based representation learning works, we can consider Diff-Rep as an application of the sufficient dimension reduction (SDR) Theorem 4 proposed from the conditional density score matching method in Sasaki and Hyvärinen 2018 [CITE].  


By Proposition 2, given that $\phi(s,a)$ and $\mu(\stil, \alpha)$ each respectively have universal approximation capability on the set of continuous functions on $S \times A$ and $S'$, then $\phi(s,a)^T\mu(\stil, \alpha)$ has universal approximation capability on $S \times A \times S'$, which represents the domain of $p(s' | s, a)$ [Cite]. [Cite that neural networks have universal approximation capability]. 

Proposition 3 follows from our above derivation of how $\phi^T \mu $ equals $\log p(s' | s, a)$ up to the partition function. Consider the desired conditional dynamics distribution $p(s' | s, a)$. 

We write:

\begin{align}
    p(s' | s, a) &\propto \exp(\phi(s,a)^T \mu(\stil, \alpha) \\
    \log p(s' | s, a) &\propto \phi(s,a)^T\mu(\stil, \alpha) \\
                    &\propto \sum_{i=1}^d \phi_{i}(s,a) \mu_{i}(\stil, \alpha)
\end{align}

where $\phi(s,a) = (\phi_{1}(s,a), \cdots, \phi_{d}(s,a))$ and $\mu(\stil, \alpha) = (\mu_{1}(\stil, \alpha), \cdots, \mu_{d}(\stil, \alpha))$

With Proposition 2 and Proposition 3 satisfied, we show how the sufficient dimension reduction framework applies to Diff-Rep. According to Sasaki and Hyvärinen 2018, SDR estimates a lower-dimensional representation of $x$ satisfying the following condition:
\begin{align}
    p(y | x) = p(y | z) \iff y \perp x|z
\end{align}
where $\perp$ represents statistical independence and $\dim z < \dim x$. 

Theorem 4 proves that if a lower dimensional representation of $z$ exists that the above condition is satisfied, $s'$ and $s,a$ are both compact, the $\log p(s' | s,a) - \log \text{partition function}$ and $\phi(s,a), \mu(\stil, \alpha) $ are continuous, and in the limit of infinite data, equations 31, 32 hold, then $\phi(s,a)$ satisfies the SDR conditions. This implies that if there exists a lower dimensional structure $z$ that can represent $x$ without loss of information, then the log conditional density can be estimated with $\dim z$ parameters instead of $\dim x$ parameters. Therefore, the $\phi(s,a)$ learned through the score-matching loss provides a low-dimensional representation of the original $S \times A$ space. We later show how this representation can be leveraged to achieve SOTA performance on standard RL benchmarks. 





\fi












\begin{algorithm}[t]
\caption{Online RL with \algabb}
\label{alg:online}
\begin{algorithmic}[1]
%\State \textbf{Input:} %Model class $\mathcal{P}=\left\{\phi(s, a) \sim p(z \mid s, a), \nabla \mu(\Tilde{s}', \alpha) \sim p\left(s^{\prime} \mid z\right))\right\}\}$,  Iteration $N$.
\State \textbf{Initialize} networks $\pi, \xi_1, \xi_2$, and $\mathcal{D} =\emptyset$ %$\pi_0(s)=\mathcal{U}(\mathcal{A})$ where $\mathcal{U}(\mathcal{A})$ denotes the uniform distribution on $\mathcal{A} ; \mathcal{D}_0=\emptyset ; \mathcal{D}_0^{\prime}=\emptyset$.

\For{timestep $t = 1 \textbf{ to } T$}
  \State $a_t \sim \pi(\cdot | s_t)$
  \State $r_t = r(s_t, a_t),\ s'_t \sim \mathbb{P}(\cdot | s_t, a_t)$
  \State Compute bonus $b(s_t, a_t)$ using \eqref{eq:bonus}  ({\emph{Optional}}) 
 % \State Collect the transition $(s_t, a_t, r_t, s'_t)$, where $a_t \sim \pi(\cdot | s_t)$, $s'_t \sim \mathbb{P}(\cdot | s,a)$, $r_t = r(s_t,a_t)$
  \State $\mathcal{D} \leftarrow \mathcal{D} \cup (s_t, a_t, r_t, s'_t)$
  % \State Update $\phi_{\theta}$ with $\mathcal{D}$  by Algorithm~\ref{alg:training} 
  \State Update the \emph{critic} $\xi_1, \xi_2$ by \eqref{eq:q-update}, alternatively
  \State Update the \emph{policy} $\pi$ by $\max_{\pi} \mathbb{E}_{s\sim \mathcal{D},a\sim\pi} [ \min_{i\in\{1,2\}} Q_{\xi_i, \theta}(s,a)]$
\EndFor

\State \textbf{Return} $\pi$.
\end{algorithmic}
\end{algorithm}






